The Bisq Decentralised Exchange: On the Privacy Cost of Participation

The Bisq Trade Protocol and the Bisq Decentralised Autonomous Organisation (DAO) are core components of Bisq, a decentralised cryptocurrency exchange. The Bisq Trade Protocol systematises the peer-to-peer trading of Bitcoin for other currencies and the Bisq DAO decentralises the governance and finance functions of the entire exchange. However, by following the Bisq Trade Protocol and interacting with the Bisq DAO, participants necessarily publish data to the Bitcoin blockchain and broadcast additional data to the Bisq peer- to-peer network. We examine the privacy cost to participants in sharing this data. Specifically, we use novel address clustering heuristics to construct the one-to-many mappings from participants to addresses on the Bitcoin blockchain and augment the address clusters with data stored within the Bisq peer-to-peer network. We describe address clustering heuristics for both the Bisq Trade Protocol and the Bisq DAO. We show that the heuristics aggregate activity performed by each participant: trading, voting, transfers, and so on. We identify instances where participants are operating under multiple aliases, some of which are real-world names. We identify the dominant transactors and their role in a two-sided market. We conclude with suggestions to better protect the privacy of participants in the future.

==> acronyms.tex <==
\newacronym{dao}{DAO}{Decentralised Autonomous Organisation}
\newacronym{roi}{RoI}{Republic of Ireland}
\newacronym{setu}{SETU}{South East Technological University}
\newacronym{utxo}{UTXO}{unspent transaction output}

